Cluster Hadronisation in Sherpa

We present the Sherpa cluster hadronization model and a simple model for non-perturbative colour reconnections. Using two different parton shower implementations we tuned the model to data and we show typical resulting distributions that are sensitive to hadronization effects in $e^+e^-$--annihilations into hadrons.

==> macros.tex <==
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{axodraw}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage{setspace}
\usepackage{threeparttable}
\usepackage{relsize}
\usepackage{ifthen}
\usepackage{lineno}
\usepackage{enumerate}
\usepackage{makeidx}
\usepackage{showidx}
\usepackage{placeins}
\setlength{\parindent}{0.0in}
\setlength{\parskip}{0.1in}

%%% Structuring
\newcommand{\Vp}{\ensuremath{\vphantom{\frac{|^|}{|^|}}}}
\newcommand{\LINE}{\underline{\hspace*{13.5cm}\hphantom{t}}\\}
\newcommand{\comment}[2][]{\noindent\LINE{\bf{#1}: }{#2}\\\LINE}
%\newcommand{\todo}[1]{\textbf{\color{red}#1}}
%\newcommand{\didit}[1]{\textbf{\color{blue}did it (#1)}}
%\newcommand{\checked}[1]{\hfill{\textbf{\color{green}\checkmark(#1)}}}
\newcommand{\todo}[1]{\fbox{\begin{minipage}{\textwidth}\textbf{#1}\end{minipage}}}
\newcommand{\didit}[1]{\textbf{\underline{#1}}}
\newcommand{\checked}[1]{\hfill{\textbf{\underline{#1}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Maths macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_maths}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Physics macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section references
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_refs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Experiments / Machines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_collabs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Software names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_codes}


\DeclareRobustCommand{\plusplus}{\raisebox{0.2ex}{\smaller++}}

\input{macros_joey}




==> macros_joey.tex <==
%\newcommand\beq{\begin{equation}}
%\newcommand\eeq{\end{equation}}
%\newcommand\beqn{\begin{eqnarray}}
%\newcommand\eeqn{\end{eqnarray}}
\newcommand\as{\alpha_S}
\newcommand\asmz{\as(M_Z^2)}
\newcommand\sighat{\hat{\sigma}}
\newcommand\GeV{{\rm GeV}}
\newcommand\MeV{{\rm MeV}}
\newcommand\qq{q \bar{q}}
\newcommand\SM{Standard Model}
%\newcommand\pp{p\bar p}
\newcommand\asQ{\as(Q^2)}
\newcommand\asm{\as(\mu^2)}
\newcommand\lmsb{\Lambda_{\overline{\rm MS}}}
\newcommand\sw{\sin{\theta_W}}
\newcommand\cw{\cos{\theta_W}}
\newcommand\stw{\sin^2{\theta_W}}
\newcommand\sttw{\sin^4{\theta_W}}
%\newcommand\c2w{\cos^2{\theta_W}}
\newcommand\lapproxeq{\lower .7ex\hbox{$\;\stackrel{\textstyle <}{\sim}\;$}}
\newcommand\gapproxeq{\lower .7ex\hbox{$\;\stackrel{\textstyle >}{\sim}\;$}}
\newcommand\TeV{{\rm TeV}}
\newcommand\la{\langle}
\newcommand\ra{\rangle}
\newcommand\qbar{\bar q}
\newcommand\ubar{\bar u}
\newcommand\dbar{\bar d}
\newcommand\bb{b\bar b}
%\newcommand\ee{e^+ e^-}
\newcommand\msb{{\overline{\rm MS}}}
\newcommand\pom{{\cal P}}
\newcommand\reg{{\cal R}}
\newcommand\cO{{\cal O}}

